A Pre-Gaia DR2 Survey for Nearby M Dwarfs in Young Associations

In this research note we identify 130 new M-type candidate members of young associations with the BANYAN $\Sigma$ tool and recently published trigonometric distances from RECONS and URAT-South. We identify a white dwarf candidate in the AB Doradus moving group, but determine that its cooling age is too large and reject it as a member. Three stars (G 13-39, LHS 2935 and G 152-1) now have complete kinematics and are strong candidate members in the AB Doradus and Carina-Near moving groups, but still lack a confirmation of their young age independent of their kinematics.

==> table_electronic.tex <==
\startlongtable
%\tabletypesize{\scriptsize}
\tabletypesize{\tiny}
%\begin{longrotatetable}
%\global\pdfpageattr\expandafter{\the\pdfpageattr/Rotate 90}
\begin{deluxetable*}{lllllr@{\;$\pm$\;}lr@{\;$\pm$\;}lr@{\;$\pm$\;}lccclllll}
\tablecolumns{19}
\tablecaption{Candidate members uncovered in this work. \label{table}}
\tablehead{\colhead{Name} & \colhead{Assoc.\tablenotemark{a}} & \colhead{Spectral} & \colhead{R.A.} & \colhead{Decl.} & \multicolumn{2}{c}{$\mu_\alpha\cos\delta$}  & \multicolumn{2}{c}{$\mu_\delta$} & \multicolumn{2}{c}{Distance} & \colhead{Rad. Vel.} & \colhead{HR1} & \colhead{$NUV$} & \colhead{IR$_{\rm ex}$} & \colhead{Known} & \colhead{Youth\tablenotemark{c}} & \colhead{Probable} & \colhead{Ref.\tablenotemark{d}}\\
\colhead{} & \colhead{} & \colhead{Type\tablenotemark{b}} & \colhead{(hh:mm:ss)} & \colhead{(dd:mm:ss)} & \multicolumn{2}{c}{($\mathrm{mas}\,\mathrm{yr}^{-1}$)} & \multicolumn{2}{c}{($\mathrm{mas}\,\mathrm{yr}^{-1}$)} & \multicolumn{2}{c}{(pc)} & \colhead{(\kms)} & \colhead{} & \colhead{(mag)} & \colhead{$N\sigma$} & \colhead{Group} & \colhead{} & \colhead{Assoc.\tablenotemark{e}} & \colhead{}
}
\startdata
LP~524--13 & ABDMG & M3 & 00:02:04.017 & +04:08:09.95 & $183.3$ & $3.3$ & $-201.4$ & $3.2$ & $22.3$ & $3.0$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG & $\cdots$ & $\cdots$ & 1,--,--,1\\
G~171--61 & ABDMG & M1.5 & 00:32:00.621 & +43:56:33.02 & $296.4$ & $3.9$ & $-268.1$ & $3.9$ & $21.5$ & $2.5$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
LP~295--636 & ABDMG & M3 & 01:12:55.574 & +27:44:51.43 & $152.3$ & $4.1$ & $-214.2$ & $4.1$ & $23.7$ & $2.9$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
G~244--32 & ABDMG & (M6) & 01:42:27.090 & +61:02:29.49 & $244.8$ & $3.1$ & $-213.2$ & $3.1$ & $23.2$ & $2.2$ & $\cdots$ & $-0.47$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 2,--,--,--\\
UCAC4~485--002908 & ABDMG & (M3) & 02:03:25.984 & +06:47:59.15 & $89.2$ & $1.2$ & $-120.5$ & $1.2$ & $23.5$ & $2.8$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG & $\cdots$ & $\cdots$ & 3,--,--,--\\
2M0203+0648 & ABDMG & (M4) & 02:03:32.320 & +06:48:57.16 & $88.4$ & $1.6$ & $-123.3$ & $1.6$ & $21.4$ & $2.4$ & $\cdots$ & $\cdots$ & $21.5 \pm 0.2$ & $\cdots$ & ABDMG & UV & $\cdots$ & --,--,--,--\\
J0210+4713 & ABDMG & (M6) & 02:10:45.383 & +47:13:24.88 & $84.6$ & $3.0$ & $-123.6$ & $3.0$ & $21.1$ & $1.7$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
LHS~1465 & ABDMG & (M6) & 02:53:07.499 & --10:19:08.53 & $354.5$ & $3.7$ & $-527.7$ & $3.5$ & $23.9$ & $2.9$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 4,--,--,--\\
G~5--12 & ABDMG & (M1) & 03:05:30.827 & +11:49:30.66 & $184.1$ & $5.9$ & $-327.3$ & $5.7$ & $23.1$ & $3.9$ & $\cdots$ & $-0.36$ & $22.2 \pm 0.4$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 5,5,5,5\\
G~5--13 & ABDMG & (M1) & 03:05:31.437 & +11:49:51.35 & $180.9$ & $6.0$ & $-326.6$ & $5.9$ & $22.5$ & $3.8$ & $\cdots$ & $-0.36$ & $20.1 \pm 0.1$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & --,--,--,--\\
G~80--14 & ABDMG & (M2) & 03:39:10.854 & +07:59:56.99 & $199.3$ & $5.1$ & $-449.6$ & $5.1$ & $21.3$ & $2.6$ & $\cdots$ & $\cdots$ & $22.1 \pm 0.4$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
LHS~5080 & ABDMG & M3.5 & 03:43:44.043 & +72:53:42.48 & $204.5$ & $3.3$ & $-437.5$ & $3.3$ & $21.1$ & $1.6$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
LHS~6062 & ABDMG & M & 03:44:50.399 & +81:53:22.76 & $231.1$ & $7.7$ & $-390.3$ & $7.4$ & $23.9$ & $3.8$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
LP~300--45 & ABDMG & (M5) & 03:49:52.994 & +30:08:48.88 & $142.3$ & $4.1$ & $-298.8$ & $3.8$ & $19.6$ & $2.6$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(92);BPMG(8) & --,--,--,6\\
LSPM~J0400+6252 & ABDMG & M & 04:00:45.494 & +62:52:42.03 & $115.9$ & $4.1$ & $-297.9$ & $3.8$ & $21.4$ & $2.2$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,6\\
LHS~1676 & ABDMG & (M7) & 04:31:44.494 & --21:50:54.66 & $452.3$ & $4.5$ & $-683.6$ & $4.2$ & $14.9$ & $1.3$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
StKM~2--388a & ABDMG & M2V & 04:50:25.486 & +19:59:09.11 & $36.2$ & $5.3$ & $-146.1$ & $5.2$ & $24.0$ & $2.8$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(84);BPMG(16) & --,--,--,--\\
Wolf~230 & ABDMG & M2V & 05:07:49.332 & +17:58:53.62 & $80.4$ & $4.8$ & $-275.5$ & $4.4$ & $9.49$ & $0.52$ & $\cdots$ & $-0.58$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(90);BPMG(10) & --,--,--,--\\
LSPM~J0521+0750 & ABDMG & (M2) & 05:21:15.254 & +07:50:23.89 & $32.8$ & $1.0$ & $-181.1$ & $1.0$ & $23.5$ & $2.5$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(90);BPMG(10) & --,--,--,--\\
LSPM~J0529+2900 & ABDMG & (M6) & 05:29:54.287 & +29:00:39.41 & $26.3$ & $3.8$ & $-172.8$ & $3.8$ & $20.3$ & $1.9$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(94);BPMG(6) & 7,--,--,--\\
LP~658--71 & ABDMG & M5 & 05:54:05.139 & --02:48:25.55 & $7.0$ & $4.1$ & $-251.4$ & $4.0$ & $18.7$ & $2.2$ & $\cdots$ & $-0.29$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
G~100--57 & ABDMG & M2.5 & 06:04:39.554 & +27:53:46.29 & $34.4$ & $3.5$ & $-373.1$ & $3.4$ & $19.8$ & $2.1$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
LP~779--34 & ABDMG & M4.0V & 06:15:11.901 & --16:26:21.23 & $-75.4$ & $2.8$ & $-373.1$ & $2.7$ & $12.89$ & $0.58$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
UCAC4~479--020861 & ABDMG & M2 & 06:31:33.816 & +05:46:48.76 & $-24.2$ & $6.5$ & $-128.9$ & $6.4$ & $22.8$ & $2.7$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(83);BPMG(15) & --,--,--,--\\
J0639-2557 & ABDMG & (M6) & 06:39:43.985 & --25:57:29.60 & $-19.10$ & $0.80$ & $-101.70$ & $0.80$ & $22.3$ & $2.4$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
UCAC4~556--032452 & ABDMG & (M1) & 06:41:33.130 & +21:11:01.97 & $-30.2$ & $4.2$ & $-156.6$ & $4.2$ & $24.0$ & $3.2$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(85);CARN(8);BPMG(7) & 8,--,--,--\\
UCAC4~493--042516 & ABDMG & (M2) & 07:18:41.870 & +08:29:59.66 & $-34.6$ & $1.3$ & $-117.4$ & $1.3$ & $24.0$ & $2.8$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 9,--,--,--\\
G~222--18 & ABDMG & M3.0Ve & 07:49:17.843 & +84:58:32.69 & $-154.2$ & $6.7$ & $-346.2$ & $6.3$ & $18.7$ & $1.8$ & $\cdots$ & $\cdots$ & $21.9 \pm 0.3$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(66);CARN(34) & --,--,--,--\\
EGGR~344 & ABDMG & DC & 07:53:27.107 & +52:29:27.45 & $-88.3$ & $6.8$ & $-256.7$ & $6.2$ & $22.0$ & $3.3$ & $\cdots$ & $\cdots$ & $18.34 \pm 0.06$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
LP~783--21 & ABDMG & M3.5 & 07:53:37.274 & --18:58:01.46 & $-129.4$ & $3.5$ & $-246.9$ & $3.5$ & $20.7$ & $1.6$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 9,--,--,--\\
UCAC3~121--75794 & ABDMG & (M3) & 08:00:53.981 & --29:33:42.39 & $-114.30$ & $0.80$ & $-94.60$ & $0.70$ & $23.4$ & $1.4$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
G~90--44 & ABDMG & M3.0Ve & 08:06:48.175 & +36:45:31.87 & $-153.7$ & $4.1$ & $-384.6$ & $3.8$ & $12.97$ & $0.84$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 10,--,--,11\\
J0835-6926 & ABDMG & (M5.5) & 08:35:12.518 & --69:26:32.04 & $-110.70$ & $0.90$ & $72.50$ & $0.90$ & $19.9$ & $2.9$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(54);BPMG(46) & 12,--,--,--\\
2M0847--5717 & ABDMG & M4 & 08:47:18.806 & --57:17:54.50 & $-128.40$ & $0.60$ & $17.70$ & $0.60$ & $23.0$ & $1.5$ & $30.2 \pm 0.2$ & $-0.04$ & $\cdots$ & $\cdots$ & ABDMG & $\cdots$ & $\cdots$ & --,--,--,--\\
G~234--57 & ABDMG & M2.5V & 09:13:23.401 & +68:52:27.09 & $-170.4$ & $5.5$ & $-231.5$ & $5.5$ & $21.0$ & $2.5$ & $\cdots$ & $-0.29$ & $19.7 \pm 0.1$ & $\cdots$ & ABDMG & UV & $\cdots$ & --,--,--,--\\
GJ~3549~B & ABDMG & M5Ve & 09:18:41.181 & +26:45:46.73 & $-182.7$ & $7.1$ & $-356.6$ & $7.1$ & $20.3$ & $3.3$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 13,--,--,--\\
LSPM~J0943+2349S & ABDMG & M1 & 09:43:01.129 & +23:49:18.39 & $-159.5$ & $5.3$ & $-220.6$ & $5.2$ & $15.2$ & $1.6$ & $\cdots$ & $\cdots$ & $21.2 \pm 0.2$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(92);COL(8) & --,--,--,--\\
LHS~2315 & ABDMG & (M8) & 10:49:12.032 & +33:31:50.48 & $-402.4$ & $6.2$ & $-446.3$ & $6.0$ & $24.1$ & $4.4$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 13,--,--,--\\
2M1104--6232 & ABDMG & (M7) & 11:04:33.295 & --62:32:35.40 & $-235.2$ & $4.0$ & $-62.0$ & $3.9$ & $17.1$ & $1.3$ & $\cdots$ & $-0.50$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
[W65]~147 & ABDMG & M3 & 11:30:18.184 & --59:59:12.57 & $-144.30$ & $0.90$ & $-64.00$ & $0.90$ & $21.8$ & $1.5$ & $\cdots$ & $-0.25$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 14,--,--,--\\
2M1145+1820 & ABDMG & M4V & 11:45:11.542 & +18:20:53.77 & $-289.4$ & $4.7$ & $-290.7$ & $4.5$ & $20.8$ & $3.0$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
J1249-4504 & ABDMG & (M5) & 12:49:54.514 & --45:04:52.96 & $-123.40$ & $0.70$ & $-112.90$ & $0.70$ & $23.1$ & $2.1$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 2,--,--,--\\
2M1257--5504 & ABDMG & (M9) & 12:57:13.028 & --55:04:03.58 & $-261.7$ & $9.2$ & $-262.0$ & $8.2$ & $16.4$ & $2.8$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 2,--,--,--\\
LHS~5238 & ABDMG & M2 & 13:06:58.121 & +27:50:53.78 & $-345.2$ & $2.8$ & $-326.7$ & $2.6$ & $22.6$ & $2.1$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 15,--,--,--\\
LP~911--25 & ABDMG & (M4) & 13:30:57.626 & --28:54:07.06 & $-221.5$ & $6.6$ & $-292.1$ & $6.5$ & $17.8$ & $1.5$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 16,--,17,18\\
UCAC3~98--145572 & ABDMG & (M7) & 14:00:49.521 & --41:09:57.35 & $-173.7$ & $4.2$ & $-196.2$ & $4.1$ & $20.1$ & $1.4$ & $\cdots$ & $-0.13$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(93);BPMG(7) & 4,--,--,--\\
LP~857--29 & ABDMG & M4.5 & 14:23:07.502 & --22:17:16.40 & $-285.5$ & $3.7$ & $-487.2$ & $3.6$ & $20.2$ & $1.9$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
Wolf~1501 & ABDMG & M3.0 & 14:41:58.913 & --16:53:17.02 & $-171.7$ & $3.4$ & $-245.0$ & $3.3$ & $22.8$ & $1.9$ & $\cdots$ & $\cdots$ & $21.8 \pm 0.4$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & --,--,--,--\\
UCAC4~262--076018 & ABDMG & (M3) & 14:50:02.521 & --37:42:15.39 & $-255.3$ & $4.5$ & $-357.4$ & $4.5$ & $23.3$ & $1.9$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(86);BPMG(14) & --,--,--,--\\
2M1511--3403 & ABDMG & (M5) & 15:11:38.355 & --34:03:24.65 & $-213.4$ & $5.5$ & $-518.1$ & $5.2$ & $21.3$ & $1.9$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
G~152--1 & ABDMG & M4.0V & 15:15:43.553 & --07:25:25.51 & $-141.0$ & $6.9$ & $-255.4$ & $6.8$ & $24.7$ & $5.6$ & $-11 \pm 2$ & $-0.22$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 3,--,--,--\\
L~264--18 & ABDMG & M2 & 15:24:48.295 & --49:29:51.30 & $-124.80$ & $0.80$ & $-242.20$ & $0.80$ & $23.5$ & $2.1$ & $10.3 \pm 0.2$ & $-0.70$ & $\cdots$ & $\cdots$ & ABDMG & $\cdots$ & $\cdots$ & 19,--,--,--\\
UCAC3~97--208389 & ABDMG & (M3) & 16:01:51.546 & --41:40:40.06 & $-45.50$ & $0.80$ & $-125.60$ & $0.80$ & $21.1$ & $1.4$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(59);BPMG(41) & 2,--,--,--\\
LHS~3216 & ABDMG & K7 & 16:34:54.875 & --53:34:48.49 & $-169.8$ & $4.5$ & $-650.5$ & $4.4$ & $15.72$ & $0.87$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(86);BPMG(14) & --,--,--,--\\
2M1637--3741 & ABDMG & (M2) & 16:37:56.297 & --37:41:34.72 & $-38.20$ & $0.70$ & $-186.20$ & $0.70$ & $23.1$ & $2.4$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(81);BPMG(19) & 3,--,--,--\\
UCAC4~216--129068 & ABDMG & MV & 16:39:25.697 & --46:53:04.88 & $-62.1$ & $5.1$ & $-287.4$ & $5.1$ & $19.2$ & $1.3$ & $\cdots$ & $-0.85$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(81);BPMG(19) & --,--,--,--\\
2M1652--2900 & ABDMG & (M5) & 16:52:35.011 & --29:00:24.45 & $-105.1$ & $6.0$ & $-365.4$ & $5.3$ & $19.4$ & $1.7$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(93);BPMG(7) & 20,--,--,--\\
UCAC4~301--127424 & ABDMG & (M5) & 17:19:19.663 & --29:49:23.40 & $-33.0$ & $4.7$ & $-514.3$ & $4.4$ & $17.6$ & $1.1$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(90);BPMG(10) & 21,22,--,22\\
LP~920--40 & ABDMG & (M4) & 17:19:20.288 & --29:49:32.04 & $-39.5$ & $4.8$ & $-520.1$ & $4.5$ & $18.6$ & $1.3$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(90);BPMG(10) & --,--,--,--\\
LP~864--14 & ABDMG & M3.5 & 17:29:46.151 & --25:04:00.79 & $-40.3$ & $2.9$ & $-464.8$ & $2.8$ & $16.64$ & $0.69$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(93);BPMG(7) & --,--,--,--\\
2M1809--0219 & ABDMG & M4.5 & 18:09:43.707 & --02:19:43.30 & $40.8$ & $7.2$ & $-542.7$ & $6.7$ & $16.9$ & $1.6$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 3,--,--,6\\
UCAC4~294--197036 & ABDMG & M4e & 18:35:21.566 & --31:23:44.27 & $20.6$ & $4.0$ & $-382.2$ & $3.8$ & $16.89$ & $0.91$ & $\cdots$ & $-0.19$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 23,--,--,--\\
UCAC4~294--197044 & ABDMG & (M6) & 18:35:22.082 & --31:23:47.87 & $22.6$ & $4.4$ & $-382.2$ & $4.3$ & $16.81$ & $0.99$ & $\cdots$ & $-0.19$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
UCAC4~280--208712 & ABDMG & (M5) & 19:03:00.581 & --34:00:17.71 & $14.4$ & $5.1$ & $-224.4$ & $5.1$ & $19.9$ & $1.6$ & $\cdots$ & $\cdots$ & $21.7 \pm 0.4$ & $\cdots$ & $\cdots$ & UV & ABDMG(95);CARN(5) & --,--,--,--\\
G~142--10 & ABDMG & (M5) & 19:09:41.779 & +09:48:52.90 & $129.6$ & $7.0$ & $-351.6$ & $6.1$ & $17.6$ & $2.8$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 3,--,--,--\\
TYC~6875--2632--1 & ABDMG & (M6) & 19:22:50.412 & --24:11:17.19 & $32.0$ & $3.6$ & $-202.4$ & $5.4$ & $20.6$ & $1.8$ & $\cdots$ & $\cdots$ & $21.5 \pm 0.5$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & 24,--,--,--\\
2M1927--0409 & ABDMG & (M7) & 19:27:13.067 & --04:09:53.22 & $60.8$ & $6.8$ & $-290.4$ & $6.4$ & $18.2$ & $1.7$ & $\cdots$ & $-0.20$ & $21.0 \pm 0.3$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & --,--,--,--\\
2M1928--3634 & ABDMG & (M6) & 19:28:33.720 & --36:34:37.10 & $94.3$ & $4.1$ & $-445.4$ & $5.8$ & $23.1$ & $2.5$ & $\cdots$ & $\cdots$ & $21.8 \pm 0.5$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & --,--,--,20\\
LP~925--27 & ABDMG & M3.0 & 19:38:27.511 & --32:31:30.69 & $88.40$ & $0.70$ & $-335.80$ & $0.70$ & $23.3$ & $2.3$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
LP~873--20 & ABDMG & (M3) & 21:14:49.618 & --22:18:47.50 & $111.5$ & $4.2$ & $-241.8$ & $4.0$ & $22.3$ & $1.8$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 15,--,--,--\\
LP~817--50 & ABDMG & M2 & 21:28:41.266 & --14:31:06.73 & $125.60$ & $0.60$ & $-190.90$ & $0.50$ & $22.9$ & $1.7$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
LP~699--32 & ABDMG & M4.4 & 22:06:09.811 & --07:23:38.00 & $169.9$ & $4.7$ & $-219.5$ & $4.7$ & $13.9$ & $1.7$ & $\cdots$ & $\cdots$ & $22.0 \pm 0.1$ & $\cdots$ & ABDMG & $\cdots$ & $\cdots$ & --,--,--,--\\
2M2253--7128 & ABDMG & (L0) & 22:53:51.763 & --71:28:09.56 & $266.5$ & $9.5$ & $-166.5$ & $8.7$ & $16.6$ & $2.7$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG(89);BPMG(9) & --,--,--,--\\
2M2317--3754 & ABDMG & (M9) & 23:17:09.169 & --37:54:51.90 & $161.8$ & $7.1$ & $-209.0$ & $7.1$ & $20.4$ & $2.6$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ABDMG & $\cdots$ & $\cdots$ & --,--,--,--\\
UCAC4~112--128210 & ABDMG & M4 & 23:25:25.744 & --67:40:10.19 & $215.2$ & $4.8$ & $-145.3$ & $4.6$ & $22.6$ & $2.1$ & $\cdots$ & $-0.47$ & $20.6 \pm 0.1$ & $\cdots$ & ABDMG & $\cdots$ & $\cdots$ & 3,--,--,--\\
L~169--58 & ABDMG & (M2) & 23:54:41.911 & --61:35:13.12 & $293.3$ & $3.9$ & $-184.7$ & $4.0$ & $17.42$ & $0.94$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
2M0004--3733 & BPMG & (M4) & 00:04:21.603 & --37:33:10.79 & $275.0$ & $4.8$ & $-147.4$ & $4.6$ & $21.9$ & $2.3$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
2M0018--8207 & BPMG & (M3) & 00:18:25.970 & --82:07:14.48 & $876.6$ & $6.8$ & $53.5$ & $6.4$ & $22.3$ & $3.6$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & BPMG(83);ABDMG(17) & 25,--,--,--\\
LP~706--97 & BPMG & (M6) & 01:05:51.039 & --11:40:39.01 & $235.6$ & $4.4$ & $-83.2$ & $4.1$ & $17.8$ & $2.7$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 15,--,--,--\\
2M0137--4558 & BPMG & M5.0 & 01:37:28.002 & --45:58:26.76 & $124.0$ & $1.1$ & $-33.0$ & $1.0$ & $20.9$ & $2.6$ & $14 \pm 1$ & $\cdots$ & $22.8 \pm 0.4$ & $\cdots$ & THA & Li,UV & $\cdots$ & --,--,--,--\\
LHS~5041 & BPMG & (M5) & 01:49:25.425 & --17:50:09.75 & $388.3$ & $4.2$ & $-243.8$ & $3.9$ & $23.5$ & $3.9$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & BPMG(63);COL(37) & 26,--,--,--\\
LP~941--90 & BPMG & (M5) & 02:28:08.335 & --36:28:20.68 & $451.6$ & $3.8$ & $-17.8$ & $3.6$ & $22.1$ & $2.0$ & $\cdots$ & $-0.30$ & $22.1 \pm 0.4$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & --,--,--,--\\
LP~711--44 & BPMG & M3 & 03:03:48.097 & --12:51:20.96 & $226.0$ & $4.0$ & $-112.2$ & $3.8$ & $18.6$ & $2.2$ & $\cdots$ & $\cdots$ & $21.8 \pm 0.1$ & $\cdots$ & $\cdots$ & UV & BPMG(84);CAR(15) & 2,--,--,--\\
LP~300--43 & BPMG & (M6) & 03:48:54.616 & +29:13:51.88 & $100.8$ & $4.9$ & $-175.4$ & $4.3$ & $24.2$ & $4.5$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & BPMG(66);ABDMG(34) & --,--,--,--\\
J0408+2008 & BPMG & (M4) & 04:08:19.734 & +20:08:29.73 & $54.0$ & $4.0$ & $-95.1$ & $4.0$ & $22.4$ & $3.2$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 27,--,--,--\\
G~8--29 & BPMG & M3.5V & 04:21:50.218 & +21:19:39.40 & $113.1$ & $5.5$ & $-228.3$ & $5.4$ & $19.2$ & $2.6$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & BPMG(57);ABDMG(43) & 23,--,--,--\\
GSC~08894--00426 & BPMG & M5Ve & 06:25:56.043 & --60:03:25.38 & $-27.20$ & $0.60$ & $117.00$ & $0.60$ & $14.20$ & $0.85$ & $\cdots$ & $-0.11$ & $\cdots$ & $\cdots$ & ABDMG & $\cdots$ & BPMG(94);ABDMG(6) & 8,28,--,--\\
J0910-4249 & BPMG & (L0) & 09:10:46.573 & --42:49:05.11 & $-179.3$ & $1.9$ & $6.6$ & $1.8$ & $19.5$ & $2.7$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 29,--,--,--\\
2M0932--4838 & BPMG & (M5) & 09:32:08.665 & --48:38:29.75 & $-247.6$ & $7.1$ & $34.1$ & $7.0$ & $23.8$ & $3.7$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & BPMG(93);COL(6) & --,--,--,--\\
CD--40~5404 & BPMG & M3V & 09:53:28 & --31:45:08 & $-148$ & $20$ & $-103$ & $20$ & $24.10$ & $0.90$ & $\cdots$ & $\cdots$ & $\cdots$ & $3.5$ & $\cdots$ & E & $\cdots$ & --,--,--,--\\
2M1145--4056 & BPMG & (M5) & 11:45:35.001 & --40:56:00.55 & $-298.9$ & $6.2$ & $-136.5$ & $6.0$ & $14.7$ & $1.1$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
UPM~J1354--7121 & BPMG & M2.5 & 13:54:53.435 & --71:21:49.75 & $-149.6$ & $3.9$ & $-129.6$ & $3.9$ & $20.0$ & $1.7$ & $3 \pm 4$ & $-0.31$ & $\cdots$ & $\cdots$ & BPMG & $\cdots$ & $\cdots$ & 4,--,--,--\\
CD--42~16413 & BPMG & M2.0 & 17:22:43 & --14:57:37 & $-50$ & $20$ & $-210$ & $20$ & $26.9$ & $1.8$ & $\cdots$ & $\cdots$ & $19.9 \pm 0.2$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & --,--,--,--\\
J1748-7427 & BPMG & (M1) & 17:48:27.703 & --74:27:58.24 & $-9.30$ & $0.60$ & $-146.80$ & $0.60$ & $20.2$ & $1.8$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & BPMG(71);ABDMG(29) & --,--,--,--\\
J1748-7427 & BPMG & (M2) & 17:48:28.080 & --74:27:43.58 & $-8.90$ & $0.80$ & $-134.7$ & $1.0$ & $19.4$ & $1.7$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & BPMG(74);ABDMG(26) & 21,30,--,22\\
UCAC4~208--168267 & BPMG & M2 & 18:00:25.918 & --48:28:28.69 & $29.2$ & $5.0$ & $-385.7$ & $4.9$ & $24.0$ & $2.4$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & BPMG(55);ABDMG(45) & --,--,--,--\\
2M1845--2337 & BPMG & $\cdots$ & 18:45:37.615 & --23:37:58.08 & $173.1$ & $4.6$ & $-547.1$ & $4.6$ & $20.0$ & $2.5$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 8,--,--,--\\
J1848-5018 & BPMG & (M3) & 18:48:15.645 & --50:18:16.96 & $56.10$ & $0.80$ & $-175.20$ & $0.80$ & $22.5$ & $2.0$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 31,31,--,--\\
J1908-3839 & BPMG & (M4) & 19:08:07.065 & --38:39:06.13 & $29.90$ & $0.60$ & $-119.90$ & $0.60$ & $22.1$ & $1.5$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 8,--,--,--\\
AU~Mic & BPMG & M1Ve & 21:27:26 & --42:15:18 & $141$ & $20$ & $-129$ & $20$ & $23.6$ & $2.0$ & $-4.5 \pm 0.3$ & $\cdots$ & $\cdots$ & $\cdots$ & BPMG & $\cdots$ & $\cdots$ & --,--,--,--\\
LP~759--6 & BPMG & (M4) & 21:57:12.862 & --09:03:28.82 & $177.6$ & $1.2$ & $-126.7$ & $1.1$ & $19.2$ & $1.6$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
Wolf~990 & BPMG & M4 & 22:06:46.852 & +03:24:58.92 & $459.3$ & $3.3$ & $-318.6$ & $3.3$ & $19.9$ & $1.5$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
LP~701--56 & BPMG & M3.0 & 23:01:46.348 & --06:14:23.95 & $175.1$ & $2.9$ & $-80.7$ & $2.9$ & $18.0$ & $1.2$ & $\cdots$ & $\cdots$ & $21.5 \pm 0.2$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & 15,28,--,--\\
LHS~6422 & BPMG & M4.0 & 23:21:56.478 & +24:12:28.77 & $409.7$ & $3.1$ & $-189.5$ & $3.1$ & $18.4$ & $2.0$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & BPMG(81);COL(19) & 32,--,--,--\\
G~273--133 & BPMG & M4.5Ve & 23:46:19.454 & --11:56:45.30 & $231.1$ & $4.8$ & $-128.3$ & $4.7$ & $18.0$ & $2.2$ & $\cdots$ & $\cdots$ & $20.81 \pm 0.06$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & 33,--,--,--\\
LHS~4038 & BPMG & M2.5 & 23:54:04.981 & --41:32:33.12 & $518.4$ & $4.5$ & $-154.0$ & $4.4$ & $24.3$ & $2.5$ & $\cdots$ & $\cdots$ & $22.4 \pm 0.3$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 21,22,--,34\\
UCAC3~65--9928 & CAR & (M5) & 04:32:57.908 & --57:41:45.59 & $71.20$ & $0.50$ & $32.40$ & $0.60$ & $18.6$ & $1.0$ & $\cdots$ & $-0.09$ & $21.9 \pm 0.3$ & $\cdots$ & $\cdots$ & UV & CAR(56);ABDMG(28);THA(16) & 15,--,--,--\\
LHS~1137 & CARN & M4.5 & 00:44:21.518 & +09:07:34.58 & $801.8$ & $5.4$ & $-10.4$ & $4.5$ & $19.0$ & $3.5$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
J0155-7026 & CARN & (M5) & 01:55:13.556 & --70:26:01.24 & $145.30$ & $0.90$ & $29.30$ & $0.90$ & $21.8$ & $3.4$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & CARN(57);BPMG(33);ABDMG(9) & --,--,--,--\\
LHS~1355 & CARN & M3.5 & 02:12:40.803 & --33:52:02.61 & $822.7$ & $5.6$ & $229.0$ & $5.0$ & $16.9$ & $1.8$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
2M0320--5536 & CARN & (M5) & 03:20:18.009 & --55:36:18.01 & $172.4$ & $4.0$ & $119.6$ & $3.5$ & $23.9$ & $2.4$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 35,--,--,--\\
LHS~1735 & CARN & (M1) & 05:06:31.819 & --29:27:07.62 & $372.3$ & $3.4$ & $418.1$ & $3.4$ & $20.2$ & $1.7$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 36,--,--,--\\
WOH~S~300 & CARN & M3.5V & 05:27:07.393 & --72:31:15.54 & $112.4$ & $5.3$ & $305.7$ & $5.2$ & $23.4$ & $3.2$ & $\cdots$ & $\cdots$ & $21.5 \pm 0.5$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & --,--,--,--\\
2M0829--5039 & CARN & (M2) & 08:29:59.807 & --50:39:32.58 & $-552.9$ & $4.6$ & $813.3$ & $4.6$ & $22.0$ & $2.1$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
Ross~688 & CARN & (M0) & 09:07:39.334 & +06:17:59.79 & $-367$ & $11$ & $-67$ & $11$ & $18.0$ & $3.0$ & $\cdots$ & $\cdots$ & $22.1 \pm 0.1$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 37,--,--,--\\
J0929-4910 & CARN & (M2) & 09:29:03.909 & --49:10:30.68 & $-152.7$ & $4.5$ & $97.20$ & $0.90$ & $22.0$ & $1.9$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 2,--,--,--\\
J1001-6814 & CARN & (M3) & 10:01:31.630 & --68:14:34.46 & $-304.1$ & $5.3$ & $202.4$ & $5.3$ & $19.9$ & $1.9$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
2M1003--2717 & CARN & (M4) & 10:03:35.763 & --27:17:44.30 & $-238.1$ & $4.1$ & $68.6$ & $4.1$ & $23.1$ & $2.1$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & ARG & $\cdots$ & $\cdots$ & --,--,--,--\\
J1005-5543 & CARN & (M5) & 10:05:45.076 & --55:43:44.23 & $-157.7$ & $1.2$ & $91.3$ & $1.4$ & $23.2$ & $3.7$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 38,--,--,--\\
G~118--51 & CARN & M3.0V & 10:20:00.206 & +28:57:09.43 & $-471.1$ & $4.1$ & $-198.6$ & $4.0$ & $19.7$ & $2.0$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 39,--,--,--\\
J1045-5059 & CARN & (M6) & 10:45:30.734 & --50:59:29.76 & $-387.3$ & $6.0$ & $116.0$ & $5.7$ & $22.0$ & $2.8$ & $\cdots$ & $-0.24$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 38,--,--,--\\
G~45--23 & CARN & (M6) & 10:58:05.453 & +06:33:46.65 & $-304.8$ & $6.2$ & $-50.7$ & $5.5$ & $24.2$ & $4.8$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
2M1058--3854 & CARN & (M6) & 10:58:46.196 & --38:54:11.62 & $-660.3$ & $6.1$ & $201.3$ & $6.0$ & $20.5$ & $2.7$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
G~56--11 & CARN & M3.5V & 11:03:08.028 & +15:17:50.42 & $-386.5$ & $6.0$ & $-95.4$ & $5.8$ & $14.8$ & $2.2$ & $\cdots$ & $-0.49$ & $20.7 \pm 0.2$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & --,--,--,--\\
LHS~5187 & CARN & (M4) & 11:05:39.020 & --52:47:14.69 & $-471.8$ & $4.9$ & $170.6$ & $4.9$ & $19.7$ & $1.8$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
LP~733--24 & CARN & M3 & 11:48:18.630 & --11:17:15.00 & $-714.4$ & $5.2$ & $-31.0$ & $5.0$ & $17.8$ & $2.8$ & $\cdots$ & $\cdots$ & $21.7 \pm 0.3$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & --,--,--,--\\
G~57--22 & CARN & (M2) & 11:49:36.889 & +17:15:40.51 & $-303.1$ & $4.9$ & $-45.3$ & $4.5$ & $23.8$ & $4.9$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
LHS~2480 & CARN & M6 & 11:57:29.003 & +79:26:59.95 & $-875.3$ & $5.6$ & $-153.8$ & $5.1$ & $18.4$ & $2.0$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & CARN(90);ABDMG(10) & --,--,--,--\\
LHS~2506 & CARN & M4 & 12:03:57.328 & --33:01:25.72 & $-755.6$ & $4.7$ & $58.0$ & $3.3$ & $19.3$ & $1.4$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
G~13--27 & CARN & K5 & 12:18:34.481 & --06:25:23.87 & $-379.5$ & $5.1$ & $-52.0$ & $4.9$ & $21.3$ & $2.2$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
LP~52--34 & CARN & M4Ve & 12:19:48.534 & --23:32:05.39 & $-222.6$ & $3.4$ & $-22.6$ & $3.4$ & $22.7$ & $2.0$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 40,--,--,--\\
G~13--39 & CARN & M3.5 & 12:27:44.384 & --03:15:01.31 & $-297$ & $10$ & $-27.4$ & $9.4$ & $21.1$ & $5.5$ & $4 \pm 3$ & $\cdots$ & $21.9 \pm 0.2$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & --,--,--,--\\
Wolf~422 & CARN & M2 & 12:32:55.137 & +12:11:32.23 & $-526.2$ & $4.9$ & $-68.4$ & $4.3$ & $19.0$ & $2.9$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 41,42,--,20\\
LHS~2608 & CARN & M3.5 & 12:42:17.157 & --71:38:20.40 & $-756.2$ & $5.0$ & $-12.4$ & $5.0$ & $13.85$ & $0.90$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 38,--,--,--\\
LHS~2935 & CARN & M6V & 14:32:08.030 & +08:11:31.34 & $-475.0$ & $4.6$ & $13.4$ & $4.5$ & $12.9$ & $1.1$ & $-18 \pm 4$ & $\cdots$ & $21.7 \pm 0.3$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 43,--,--,--\\
LHS~3022 & CARN & M4.5 & 15:04:57.556 & --21:07:03.80 & $-657.8$ & $1.0$ & $-199.6$ & $1.0$ & $18.6$ & $1.3$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 23,--,--,20\\
UCAC3~123--175263 & CARN & M5 & 15:16:52.075 & --28:32:21.33 & $-852.3$ & $6.0$ & $-314.1$ & $5.4$ & $21.5$ & $2.1$ & $\cdots$ & $\cdots$ & $20.2 \pm 0.2$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & 29,--,--,--\\
LHS~3057 & CARN & M3 & 15:19:17.383 & +67:51:23.69 & $-465.8$ & $2.5$ & $402.0$ & $2.5$ & $21.1$ & $1.8$ & $\cdots$ & $\cdots$ & $21.5 \pm 0.5$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & --,--,--,--\\
G~179--55 & CARN & M4.0V & 15:47:26.994 & +45:07:54.83 & $-253.1$ & $2.8$ & $200.3$ & $2.8$ & $20.5$ & $1.7$ & $\cdots$ & $-1.00$ & $20.6 \pm 0.2$ & $\cdots$ & $\cdots$ & UV & $\cdots$ & --,--,--,--\\
LHS~3793 & CARN & M4.5 & 22:19:24.680 & --28:23:24.58 & $859.1$ & $3.8$ & $-251.9$ & $3.8$ & $18.0$ & $1.4$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 8,--,--,--\\
G~33--6 & COL & M3.5Ve & 00:44:19.631 & +12:36:59.87 & $284.7$ & $1.6$ & $-182.1$ & $1.5$ & $15.6$ & $1.7$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & COL(56);BPMG(44) & --,--,--,20\\
SCR~J0150--3741 & COL & (M5) & 01:50:13.503 & --37:41:53.45 & $191.3$ & $6.1$ & $-78.1$ & $6.0$ & $14.8$ & $1.2$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & COL(51);CAR(37);BPMG(11) & 8,--,--,--\\
G~246--35 & COL & (M6) & 03:26:31.387 & +59:08:50.73 & $179.5$ & $3.4$ & $-191.7$ & $3.3$ & $21.6$ & $1.9$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 44,--,--,20\\
LSPM~J0701+1558 & COL & (M7) & 07:01:10.672 & +15:58:25.09 & $-10.4$ & $5.0$ & $-187.5$ & $4.9$ & $20.8$ & $2.6$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & COL(79);ABDMG(21) & 23,--,--,--\\
HG~7--141 & HYA & M2 & 04:16:03.706 & +18:51:32.64 & $112.1$ & $3.5$ & $-34.2$ & $3.4$ & $23.3$ & $2.4$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & HYA & $\cdots$ & $\cdots$ & 29,--,--,--\\
J1344+5528 & UMA & (M6) & 13:44:58.087 & +55:28:21.54 & $111.5$ & $3.1$ & $-28.7$ & $3.0$ & $24.0$ & $2.6$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & --,--,--,--\\
\enddata
\tablenotetext{a}{Young association: AB~Doradus moving group (ABDMG), $\beta$~Pictoris moving group (BPMG), CAR (Carina), CARN (Carina-Near), COL (Columba), HYA (Hyades) or UMA (Ursa Major moving group). See \cite{2018ApJ...856...23G} for more detail.}
\tablenotetext{b}{Spectral types in parentheses were estimated using the $G - J$ color with the spectral type--color relations of \cite{2013ApJS..208....9P}, see also \url{http://www.pas.rochester.edu/~emamajek/EEM_dwarf_UBVIJHK_colors_Teff.txt}.}
\tablenotetext{c}{Signs of youth compiled from the literature. See J.~Gagn\'e, O.~Loublier, J.~K.~Faherty et al. (submitted to ApJ) for more detail. X: X-ray emission with HR1 $\geq$ -0.15; UV: Galex $NUV-G$ versus $G-J$ consitent with youth; Li: Lithium absorption above 100\,m\AA; E: Mid-infrared excess.}
\tablenotetext{d}{References for: (1) spectral type, (2) radial velocity, (3) lithium equivalent width and (4) membership candidacy in a young association.}
\tablenotetext{e}{Possible young associations are listed with the corresponding relative probabilities (\%) in parenthesis.}
\tablerefs{(1)~\citealt{2015ApJS..219...33G}; (2)~\citealt{2004AJ....128..463R}; (3)~\citealt{2013AJ....145..102L}; (4)~\citealt{2015RAA....15.1154Z}; (5)~\citealt{2014AJ....147..146K}; (6)~\citealt{2012AJ....143...80S}; (7)~\citealt{2016ApJ...817....1J}; (8)~\citealt{2005AA...442..211S}; (9)~\citealt{2018AJ....155..176F}; (10)~\citealt{1968ApJ...151..605P}; (11)~\citealt{2011AA...531A..92R}; (12)~\citealt{2017AA...597A..47C}; (13)~\citealt{1986AJ.....92..139S}; (14)~\citealt{2007AJ....133.2898F}; (15)~\citealt{2015AA...577A.128A}; (16)~\citealt{1997AJ....114..244C}; (17)~\citealt{2009AA...508..833D}; (18)~\citealt{2004ARAA..42..685Z}; (19)~\citealt{2013ApJS..204....5K}; (20)~\citealt{2015ApJ...798...73G}; (21)~\citealt{2006AJ....132..866R}; (22)~\citealt{2014ApJ...788...81M}; (23)~\citealt{2003AJ....126.3007R}; (24)~\citealt{2002AJ....123.2002H}; (25)~\citealt{1965MNRAS.130...45W}; (26)~\citealt{2017AJ....154...67M}; (27)~\citealt{2001KFNT...17..409K}; (28)~\citealt{2017AJ....153...75K}; (29)~\citealt{1985ApJS...59..197B}; (30)~\citealt{RAVE}; (31)~\citealt{2014AJ....147...20N}; (32)~\citealt{2016ApJS..224...36K}; (33)~\citealt{1995AJ....110.1838R}; (34)~\citealt{2013ApJ...762...88M}; (35)~\citealt{2014AA...568A..54R}; (36)~\citealt{2014ApJ...787..126L}; (37)~\citealt{2010MNRAS.403.1949K}; (38)~\citealt{2014MNRAS.443.2561G}; (39)~\citealt{2003AJ....125.1598L}; (40)~\citealt{2007AJ....133.2825R}; (41)~\citealt{1989ApJS...71..245K}; (42)~\citealt{2011AAS...21743412C}; (43)~\citealt{2016MNRAS.457.2192C}; (44)~\citealt{2013AA...556A..15R}.}
\end{deluxetable*}
\end{longrotatetable}
\global\pdfpageattr\expandafter{\the\pdfpageattr/Rotate 0}
